Understanding Cross-Lingual Syntactic Transfer in Multilingual Recurrent Neural Networks

It is now established that modern neural language models can be successfully trained on multiple languages simultaneously without changes to the underlying architecture. But what kind of knowledge is really shared among languages within these models? Does multilingual training mostly lead to an alignment of the lexical representation spaces or does it also enable the sharing of purely grammatical knowledge? In this paper we dissect different forms of cross-lingual transfer and look for its most determining factors, using a variety of models and probing tasks. We find that exposing our LMs to a related language does not always increase grammatical knowledge in the target language, and that optimal conditions for lexical-semantic transfer may not be optimal for syntactic transfer.

==> agreement_eg.tex <==
\begin{tkzcd}
The boys & 
\end{tkzcd}


==> agreement_new.tex <==
% Created by tikzDevice version 0.12.3.1 on 2021-02-09 10:35:58
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,180.67);
\begin{scope}
\path[clip] ( 28.32, 16.64) rectangle (119.82,152.62);
\definecolor{fillColor}{gray}{0.67}

\path[fill=fillColor] ( 30.61,-125.13) rectangle ( 38.85, 32.90);

\path[fill=fillColor] ( 76.36,-125.13) rectangle ( 84.59, 31.72);
\definecolor{fillColor}{gray}{0.35}

\path[fill=fillColor] ( 63.55,-125.13) rectangle ( 71.78,125.28);

\path[fill=fillColor] (109.30,-125.13) rectangle (117.53,104.54);
\definecolor{fillColor}{RGB}{0,107,164}

\path[fill=fillColor] ( 38.85,-125.13) rectangle ( 47.08,105.84);

\path[fill=fillColor] ( 84.59,-125.13) rectangle ( 92.83,104.54);
\definecolor{fillColor}{RGB}{255,140,0}

\path[fill=fillColor] ( 47.08,-125.13) rectangle ( 55.31, 91.26);

\path[fill=fillColor] ( 92.83,-125.13) rectangle (101.06, 84.37);
\definecolor{fillColor}{RGB}{205,102,0}

\path[fill=fillColor] ( 55.31,-125.13) rectangle ( 63.55,125.95);

\path[fill=fillColor] (101.06,-125.13) rectangle (109.30,108.47);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at ( 34.73, 33.20) {$54.6$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at ( 80.48, 32.01) {$54.2$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at ( 67.67,125.58) {$86.6$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (113.41,104.83) {$79.4$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at ( 42.96,106.13) {$79.8$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at ( 88.71,104.83) {$79.4$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at ( 51.20, 91.55) {$74.8$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at ( 96.94, 84.67) {$72.4$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at ( 59.43,126.24) {$86.8$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (105.18,108.77) {$80.7$};
\end{scope}
\begin{scope}
\path[clip] (119.82, 16.64) rectangle (211.31,152.62);
\definecolor{fillColor}{gray}{0.67}

\path[fill=fillColor] (122.10,-125.13) rectangle (130.34, 48.32);

\path[fill=fillColor] (167.85,-125.13) rectangle (176.09, 30.91);
\definecolor{fillColor}{gray}{0.35}

\path[fill=fillColor] (155.04,-125.13) rectangle (163.28,139.92);

\path[fill=fillColor] (200.79,-125.13) rectangle (209.02,126.82);
\definecolor{fillColor}{RGB}{0,107,164}

\path[fill=fillColor] (130.34,-125.13) rectangle (138.57,130.20);

\path[fill=fillColor] (176.09,-125.13) rectangle (184.32,105.84);
\definecolor{fillColor}{RGB}{255,140,0}

\path[fill=fillColor] (138.57,-125.13) rectangle (146.81,128.12);

\path[fill=fillColor] (184.32,-125.13) rectangle (192.55,101.27);
\definecolor{fillColor}{RGB}{205,102,0}

\path[fill=fillColor] (146.81,-125.13) rectangle (155.04,136.48);

\path[fill=fillColor] (192.55,-125.13) rectangle (200.79,103.44);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (126.22, 48.62) {$60$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (171.97, 31.20) {$53.9$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (159.16,140.22) {$91.6$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (204.91,127.11) {$87.1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (134.46,130.49) {$88.2$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (180.20,106.13) {$79.8$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (142.69,128.41) {$87.5$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (188.44,101.56) {$78.2$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (150.92,136.77) {$90.4$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.43] at (196.67,103.73) {$79$};
\end{scope}
\begin{scope}
\path[clip] ( 28.32,152.62) rectangle (119.82,175.17);
\definecolor{drawColor}{gray}{0.10}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 74.07,165.26) {\bfseries FR$\rightarrow$IT};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 74.07,157.70) {\bfseries ES$\rightarrow$IT};
\end{scope}
\begin{scope}
\path[clip] (119.82,152.62) rectangle (211.31,175.17);
\definecolor{drawColor}{gray}{0.10}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (165.56,165.26) {\bfseries FR$\rightarrow$RU};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (165.56,157.70) {\bfseries UK$\rightarrow$RU};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 28.32, 16.64) --
	(119.82, 16.64);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 51.20,  6.86) {\bfseries Original};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 96.94,  6.86) {\bfseries Nonce};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] (119.82, 16.64) --
	(211.31, 16.64);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (142.69,  6.86) {\bfseries Original};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.70] at (188.44,  6.86) {\bfseries Nonce};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 28.32, 16.64) --
	( 28.32,152.62);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 23.37, 17.12) {\bfseries 50};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 23.37, 46.05) {\bfseries 60};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 23.37, 74.98) {\bfseries 70};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 23.37,103.92) {\bfseries 80};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.70] at ( 23.37,132.85) {\bfseries 90};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 11.02, 84.63) {\bfseries Accuracy};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{fillColor}{gray}{0.67}

\path[fill=fillColor] ( 42.20,139.31) rectangle ( 55.23,152.34);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{fillColor}{RGB}{0,107,164}

\path[fill=fillColor] ( 72.30,139.31) rectangle ( 85.33,152.34);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{fillColor}{RGB}{255,140,0}

\path[fill=fillColor] (100.92,139.31) rectangle (113.96,152.34);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{fillColor}{RGB}{205,102,0}

\path[fill=fillColor] (138.38,139.31) rectangle (151.41,152.34);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{fillColor}{gray}{0.35}

\path[fill=fillColor] (176.46,139.31) rectangle (189.49,152.34);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.45] at ( 58.79,144.27) {Freq.};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.45] at ( 88.88,146.70) {IT$_s$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.45] at ( 88.88,141.84) {RU$_s$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.45] at (117.51,146.70) {FR$\rightarrow$IT};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.45] at (117.51,141.84) {FR$\rightarrow$RU};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.45] at (154.97,146.70) {ES$\rightarrow$IT};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.45] at (154.97,141.84) {UK$\rightarrow$RU};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.45] at (193.04,146.70) {IT$_l$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.45] at (193.04,141.84) {RU$_l$};
\end{scope}
\end{tikzpicture}


==> pos_new.tex <==
% Created by tikzDevice version 0.12.3 on 2019-11-27 13:55:30
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] ( 37.01, 18.22) rectangle (121.41,155.44);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 37.01, 40.05) --
	(121.41, 40.05);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 37.01, 71.24) --
	(121.41, 71.24);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 37.01,102.42) --
	(121.41,102.42);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 37.01,133.61) --
	(121.41,133.61);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 37.01, 24.46) --
	(121.41, 24.46);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 37.01, 55.65) --
	(121.41, 55.65);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 37.01, 86.83) --
	(121.41, 86.83);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 37.01,118.02) --
	(121.41,118.02);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 37.01,149.20) --
	(121.41,149.20);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 49.07, 18.22) --
	( 49.07,155.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 69.16, 18.22) --
	( 69.16,155.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 89.26, 18.22) --
	( 89.26,155.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (109.35, 18.22) --
	(109.35,155.44);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] ( 49.07, 24.46) rectangle ( 58.11,145.08);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] ( 40.03, 24.46) rectangle ( 49.07,146.37);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] ( 69.16, 24.46) rectangle ( 78.21,104.56);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] ( 60.12, 24.46) rectangle ( 69.16,107.20);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] ( 89.26, 24.46) rectangle ( 98.30,143.88);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] ( 80.22, 24.46) rectangle ( 89.26,143.83);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] (109.35, 24.46) rectangle (118.40,105.46);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] (100.31, 24.46) rectangle (109.35,106.03);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 53.59,145.65) {96.69};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 44.55,146.93) {97.72};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 73.68,105.13) {64.21};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 64.64,107.76) {66.32};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 93.78,144.44) {95.73};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at ( 84.74,144.40) {95.69};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (113.87,106.03) {64.93};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (104.83,106.60) {65.39};
\end{scope}
\begin{scope}
\path[clip] (126.91, 18.22) rectangle (211.31,155.44);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.3pt,line join=round] (126.91, 40.05) --
	(211.31, 40.05);

\path[draw=drawColor,line width= 0.3pt,line join=round] (126.91, 71.24) --
	(211.31, 71.24);

\path[draw=drawColor,line width= 0.3pt,line join=round] (126.91,102.42) --
	(211.31,102.42);

\path[draw=drawColor,line width= 0.3pt,line join=round] (126.91,133.61) --
	(211.31,133.61);

\path[draw=drawColor,line width= 0.6pt,line join=round] (126.91, 24.46) --
	(211.31, 24.46);

\path[draw=drawColor,line width= 0.6pt,line join=round] (126.91, 55.65) --
	(211.31, 55.65);

\path[draw=drawColor,line width= 0.6pt,line join=round] (126.91, 86.83) --
	(211.31, 86.83);

\path[draw=drawColor,line width= 0.6pt,line join=round] (126.91,118.02) --
	(211.31,118.02);

\path[draw=drawColor,line width= 0.6pt,line join=round] (126.91,149.20) --
	(211.31,149.20);

\path[draw=drawColor,line width= 0.6pt,line join=round] (138.97, 18.22) --
	(138.97,155.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (159.06, 18.22) --
	(159.06,155.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (179.16, 18.22) --
	(179.16,155.44);

\path[draw=drawColor,line width= 0.6pt,line join=round] (199.25, 18.22) --
	(199.25,155.44);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] (138.97, 24.46) rectangle (148.01,143.44);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] (129.92, 24.46) rectangle (138.97,145.17);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] (159.06, 24.46) rectangle (168.11, 89.17);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] (150.02, 24.46) rectangle (159.06, 29.20);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] (179.16, 24.46) rectangle (188.20,143.89);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] (170.11, 24.46) rectangle (179.16,143.74);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] (199.25, 24.46) rectangle (208.30, 92.12);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] (190.21, 24.46) rectangle (199.25, 30.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (143.49,144.01) {95.38};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (134.45,145.74) {96.77};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (163.58, 89.74) {51.88};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (154.54, 29.77) {3.8};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (183.68,144.46) {95.74};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (174.64,144.31) {95.62};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (203.77, 92.68) {54.24};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.83] at (194.73, 31.11) {4.88};
\end{scope}
\begin{scope}
\path[clip] ( 37.01,155.44) rectangle (121.41,174.86);
\definecolor{drawColor}{gray}{0.10}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.20] at ( 79.21,161.01) {\bfseries Joint Training};
\end{scope}
\begin{scope}
\path[clip] (126.91,155.44) rectangle (211.31,174.86);
\definecolor{drawColor}{gray}{0.10}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.20] at (169.11,161.01) {\bfseries Pre-Training};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 49.07,  7.21) {$FR\rightarrowFR$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 69.16,  7.21) {$IT\rightarrowFR$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 89.26,  7.21) {$IT\rightarrowIT$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (109.35,  7.21) {$FR\rightarrowIT$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (138.97,  7.21) {FR->FR};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (159.06,  7.21) {IT->FR};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (179.16,  7.21) {IT->IT};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (199.25,  7.21) {FR->IT};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 32.06, 21.43) {0};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 32.06, 52.61) {25};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 32.06, 83.80) {50};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 32.06,114.99) {75};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 32.06,146.17) {100};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.20] at ( 13.78, 86.83) {\bfseries Accuracy};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 18.87,194.79) {\bfseries Vocabulary Overlap};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] (135.36,192.07) rectangle (148.39,205.10);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] (180.61,192.07) rectangle (193.64,205.10);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.88] at (154.60,195.55) {None};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.88] at (199.85,195.55) {Natural};
\end{scope}
\end{tikzpicture}


==> word-translation.tex <==
% Created by tikzDevice version 0.12.3 on 2019-11-27 14:28:52
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] ( 19.25, 29.82) rectangle (112.53,157.21);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] ( 36.74, 35.61) rectangle ( 49.86,114.58);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] ( 23.62, 35.61) rectangle ( 36.74,103.68);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] ( 65.89, 35.61) rectangle ( 79.01,143.76);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] ( 52.77, 35.61) rectangle ( 65.89,138.40);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] ( 95.04, 35.61) rectangle (108.16,151.42);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] ( 81.92, 35.61) rectangle ( 95.04,149.32);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at ( 42.92,114.92) {55.25};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at ( 28.35,104.01) {47.62};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at ( 72.07,144.09) {75.66};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at ( 57.50,138.73) {71.91};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at (101.22,151.75) {81.02};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at ( 86.65,149.65) {79.55};
\end{scope}
\begin{scope}
\path[clip] (118.03, 29.82) rectangle (211.31,157.21);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] (135.52, 35.61) rectangle (148.64, 35.62);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] (122.40, 35.61) rectangle (135.52, 87.57);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] (164.67, 35.61) rectangle (177.79, 35.71);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] (151.55, 35.61) rectangle (164.67,123.55);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] (193.82, 35.61) rectangle (206.94, 35.81);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] (180.70, 35.61) rectangle (193.82,137.30);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at (141.95, 35.95) {0.01};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at (127.13, 87.90) {36.35};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at (171.10, 36.04) {0.07};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at (156.28,123.88) {61.52};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at (200.25, 36.14) {0.14};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.48] at (185.43,137.63) {71.14};
\end{scope}
\begin{scope}
\path[clip] ( 19.25,157.21) rectangle (112.53,174.86);
\definecolor{drawColor}{gray}{0.10}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 65.89,162.58) {\bfseries Joint Training};
\end{scope}
\begin{scope}
\path[clip] (118.03,157.21) rectangle (211.31,174.86);
\definecolor{drawColor}{gray}{0.10}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (164.67,162.58) {\bfseries Pre-Training};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 19.25, 29.82) --
	(112.53, 29.82);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 36.74, 18.81) {\textbf{P\\@1}};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 65.89, 18.81) {\textbf{P\\@5}};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 95.04, 18.81) {\textbf{P\\@10}};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] (118.03, 29.82) --
	(211.31, 29.82);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (135.52, 18.81) {\textbf{P\\@1}};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (164.67, 18.81) {\textbf{P\\@5}};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (193.82, 18.81) {\textbf{P\\@10}};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 19.25, 29.82) --
	( 19.25,157.21);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 14.30, 32.58) {0};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 14.30, 61.17) {20};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 14.30, 89.75) {40};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 14.30,118.34) {60};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 14.30,146.93) {80};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (115.28,  7.44) {\bfseries Precision};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 16.00,195.13) {\bfseries Vocabulary Overlap};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{fillColor}{RGB}{102,194,165}

\path[fill=fillColor] (121.97,192.07) rectangle (135.00,205.10);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{fillColor}{RGB}{252,141,98}

\path[fill=fillColor] (176.02,192.07) rectangle (189.05,205.10);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.88] at (140.71,195.55) {Natural};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.88] at (194.76,195.55) {None};
\end{scope}
\end{tikzpicture}

